Estimating the Impact of Wind Generation in the UK

This paper studies the impact of wind generation on market prices and system costs in the UK between 2013 and 2014. The wider effects and implications of wind generation is of direct relevance and importance to policy makers, as well as the grid operator and market traders. We compare electricity generation from Coal, Gas and wind, on both the wholesale and imbalance market. We calculate the system cost of wind generation (government subsidies and curtailment costs) and the total energy costs. For the first time in the UK, we calculate the Merit Order Effect on spot price due to the wind component and show a $1.67\%$ price decrease for every percentage point of wind generation (compared to the ``zero-wind'' price). The net result of total costs and price savings is roughly zero (slight positive gain). We also consider the effect of not having either an onshore or an offshore wind component. We show that the Merit-Order Effect savings are heavily reduced, leading to an outgoing cost of wind generation in both cases. It is therefore important to have a significant total percentage of wind generation, from both onshore and offshore farms.

==> tables/table_data_sources.tex <==
\begin{table}[]
\centering
\scriptsize
\begin{tabular}{|l|l|ll|}
\hline
\textbf{Data set}                     & \textbf{Source}            & \textbf{Start Date} & \textbf{End Date} \\ \hline
\textbf{Generation by Fuel Type} & Elexon Portal   & 01/08/2012               & 18/03/2015             \\
\textbf{Spot Price}              & APX Group          & 16/06/2008               & 09/08/2015             \\ 
\textbf{Balancing Mechanism}               & BM Reports         & 01/08/2012               & 18/03/2015             \\ \hline
\end{tabular}
\caption{Data sources utilised in the analysis and relevant date ranges.}
\label{tab:data_sources}
\end{table}
